CATERPILLAR: Coarse Grain Reconfigurable Architecture for Accelerating the Training of Deep Neural Networks

Accelerating the inference of a trained DNN is a well studied subject. In this paper we switch the focus to the training of DNNs. The training phase is compute intensive, demands complicated data communication, and contains multiple levels of data dependencies and parallelism. This paper presents an algorithm/architecture space exploration of efficient accelerators to achieve better network convergence rates and higher energy efficiency for training DNNs. We further demonstrate that an architecture with hierarchical support for collective communication semantics provides flexibility in training various networks performing both stochastic and batched gradient descent based techniques. Our results suggest that smaller networks favor non-batched techniques while performance for larger networks is higher using batched operations. At 45nm technology, CATERPILLAR achieves performance efficiencies of 177 GFLOPS/W at over 80% utilization for SGD training on small networks and 211 GFLOPS/W at over 90% utilization for pipelined SGD/CP training on larger networks using a total area of 103.2 mm$^2$ and 178.9 mm$^2$ respectively.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> abstract_1.tex <==
\begin{abstract}
%With the increasing popularity of DNNs and CNNs several efforts have focused on the architectural studies and implementation of the feed forward/inference of a trained network. In this paper we switch the focus to training of deep neural networks. 
This paper presents an algorithm/architecture space exploration of efficient accelerators for training deep neural networks. We demonstrate the interplay between architectural choices and algorithmic techniques to achieve better network convergence rates and higher energy efficiency.  We further demonstrate that an architecture with hierarchical support for collective communication semantics provides flexibility in training various networks using both batched and non-batched techniques. Our results suggest that smaller networks favor non-batched techniques like continuous propagation while performance for larger networks is higher using batched operations.  At 45nm technology, we are able to achieve performance efficiencies of 407GFLOPs/W for non-minibatched learning on small networks and 780GFLOPs/W for minibatched learning on larger networks.
\end{abstract}

==> abstract__Ardavan_Pedram_s_conflicted_copy_2017-04-05_.tex <==
\begin{abstract}
With the increasing popularity of DNNs and CNNs  have focused on the architectural studies and implementation of the feed forward/inference of a trained network. In this paper we switch the focus to training of deep neural networks. 
This paper presents an algorithm/architecture space exploration of efficient accelerators for training deep neural networks. We demonstrate the interplay between architectural choices and algorithmic techniques to achieve better network convergence rates and higher energy efficiency.  We further demonstrate that an architecture with hierarchical support for collective communication semantics provides flexibility in training various networks using both batched and non-batched techniques. Our results suggest that smaller networks favor non-batched techniques like continuous propagation while performance for larger networks is higher using batched operations.  At 45nm technology, we are able to achieve performance efficiencies of 407GFLOPs/W for non-minibatched learning on small networks and 780GFLOPs/W for minibatched learning on larger networks.
\end{abstract}

==> arch_ardavan.tex <==
\section{Architecture}

In this section we describe architecture design and tradeoffs for various networks sizes and describe 
 how computation/communication and parallelism tradeoffs affect our design.



\begin{figure*}[tb]
\centering
\includegraphics[width=.9 \textwidth]{Arch}
\vspace{-10pt}
\caption{Multi-core Architecture }
\label{fig:learning}
\end{figure*}




\subsection{Discussion of Various Algorithms with Respect to Locality and Parallelism}

The nature of operation in each layer of Neural Network is Matrix Vector Multilpication as shown in figure\ref{}.
\P{we can assume here there two cases 1- Network fits in local memories  2- it does not fit. But we have not yet introduced the architecture.}
\begin{enumerate}
\item
\AP{locality for weights}
For continuous propagation and the GEMV architecture, there is locality within the inputs as each input layer is multiplied by multiple weights.
\item
\AP{locality for activation}
As seen in the MLP derivation, the activations, $h_i$, computed during the forward pass are needed in the backward pass to update the weights.  Consequently, there is locality between the forward and backward pass, requiring us to store the activations.  However, layers are visited in the reverse order during backpropagation so that for a single sample, the first activation to be produced is the last one to be consumed.  The last layer's activation is used immediately, the second last layer's activation is stored for the duration of the forward/backward pass of the last layer, the third last layer's activation is stored for the duration of the forward/backward pass of the last two layers, and so on.  For stochastic gradient descent and continuous propagation, a small number of samples go through the network at a time so that the size of the activation at each layer is considerably smaller than the weights.  In this case, we can simply store all the activations without incurring much memory overhead compared to the memory required for the weights.  While activation size is still smaller than weight size for batched gradient descent, as the network grows deeper, the total size of activations to be stored is on the order of magnitude of the weights and the memory overhead becomes a concern.  To mitigate this we can use reverse checkpointing, which only saves the activations for some layers.  During backpropagation when we need an activation that has not been saved, we go back to the last saved activation for that input and go through the forward path again to recalculate the activation we need.
\item \AP{Locality within samples}
This is mini batching the algorithms so they look like GEMM operations.
\end{enumerate}

\subsection{GEMV (if it fits)}

The GEMV friendly architecture is designed for use with stochastic gradient descent and continuous propagation as it is just a series of matrix-vector multiplications.  The core is an array of processing elements (PEs) with buses for broadcasting between columns and rows.  To compute the matrix-vector multiplication we distribute the weights to the array of PEs in 2D round robin fashion and broadcast the input vector to the layer across the column buses.  We then perform a reduction across each row of PEs to obtain the output vector, storing the results on the diagonal PEs to allow easy calculation of the transpose during backpropagation.  

The arrangement of the PE array determines the cost of broadcasts and reductions for a layer.  In particular, a wide PE array will have faster broadcasts but require more reductions while the opposite is true for a tall array.  However, broadcasts and reductions are reversed during backpropagation - to optimize broadcast vs. reduction costs we choose a square PE array.

To produce an output vector of size n from an input vector of size n, we need to use $n^2$ weights, thus consumption rate of weights is $n^2$ while consumption/production rate of activations is only $n$.  If the weights do not fit on the core and we need to bring them in from off-core memory, then we require high memory bandwidth in order to provide weights fast enough to the core.  Ideally, we want the on-core memory to be large enough that the weights can all fit on the core.

For large networks that do not fit on one core, we can divide layers between cores proportional to the number of calculations needed to calculate an output for each layer and store the weights on the cores.  If the network weights are too large to fit on an array of cores, we can store as many layer weights as possible on the cores, starting from the last layer.  We choose to store the last layers because of the temporal locality introduced by the fact that the last weights used during forward propagation are the first weights used/updated during backpropagation.

Besides storing the weights for each layer we also need to store the input and the activation for the layer for use during backpropagation.  When computing the output, we can either work on the same portion of the output and cycle through the inputs multiple times, once for each portion, or work on all portions of the output and go through the inputs only once.  Thus we also need to store the partial sums of the output locally on the PEs.  

Suppose we have a network with L layers with cores that have $n_r^2$ PEs.  Then for the ith layer of size m x n, mapped to a*b cores, the memory needed per PE for this layer is:

\begin{align*}
(L-i+1)\frac{m+n}{abn_r^2} + \frac{max(m,n)}{max(a,b)n_r} + \frac{mn}{abn_r^2}
\end{align*}

\subsection{GEMM}

The GEMM friendly architecture is designed for use with minibatch gradient descent/continuous propagation.  Once again, each core is an array of PEs and we can use multiple cores per layer.  However the input here is a matrix rather than a vector.  Matrix-matrix multiplication can be done using outer products between the inputs and the weights, with each outer product producing a portion of the matrix output.  To produce an $n_r^2$ block of output partial sums, we need a length $n_r$ column of the weights and a length $n_r$ row of the inputs.  Note that unlike the GEMV architecture, the bandwidth required to bring in weights from off-core memory is linear rather than quadratic with respect to the problem size.  Consequently, it is not necessary to be able to store all of the weights on-core, although the size of the inputs and activations we need to store is greater.  

For the ith layer, the memory needed per PE for minibatch of size k is:

\begin{align*}
(j-i+1)\frac{k(m+n)}{abn_r^2}
\end{align*}

where j is the index of the previous layer checkpointed and layer i is checkpointed.  If layer i is not checkpointed, then we recalculate rather than store the activations and the required memory per PE is:

\begin{align*}
\frac{k(m+n)}{abn_r^2}
\end{align*}

\subsection{Computations}

\subsubsection{Multiply Accumulate}

Regardless of the learning method or architecture chosen, the number of multiply-accumulate (MAC) operations required is the same in the forward pass.  For a single epoch over a dataset of size $K$ and a network with $L$ layers, the number of MACs required is:

\begin{align*}
\sum\limits_{i=1}^LKm_in_i
\end{align*}

where the ith layer is size $m_i \times n_i$

During backpropagation, the number of MAC operations depends on the learning method chosen.  For SGD, BGD, CP, and FA, assuming we store all required activations, the number of MAC operations to backpropagate the errors are:

\begin{align*}
\sum\limits_{i=2}^LKm_in_i
\end{align*}

Note that the summation excludes the first layer, since we do not need to propagate its error.

For DFA, we propagate the last layer's error to all layers and so the number of MAC operations are:

\begin{align*}
\sum\limits_{i=2}^LKm_in_L
\end{align*}

Here the ith layer has inputs of size $m_i$ and the output of the network is size $n_L$

In order to calculate the weight gradients for all learning methods, the number of MAC operations are:

\begin{align*}
\sum\limits_{i=1}^LKm_in_i
\end{align*}

Note that although the number of weight updates that occur per epoch is different depending on the minibatch size, the total number of MAC operations to calculate the gradients is the same.

If we use checkpointing rather than storing all activations, the number of MACs required increases as we must reiterate through parts of the forward path during backpropagation.  For layer $i$ that has not had its activations stored, the number of MAC operations during recalculation is:

\begin{align*}
\sum\limits_{j=c}^iKm_jn_j
\end{align*}

where layer c is the previous layer to have its activations stored.

\subsubsection{Weight Accesses}

We need to access each weight once during forward propagation and once during backpropagation/weight updates.  The number of weight accesses is dependent on the minibatch size.  For minibatch size of $b$, the number of weight accesses per epoch is:

\begin{align*}
2\sum\limits_{i=2}^L\frac{K}{b}m_in_i + \frac{K}{b}m_1n_1
\end{align*}

\subsection{Precision}

Our baseline models are trained 16bit floating point (no discernible difference was found between using 16bit and 32bit floating point).  Gupta et al. show that for a 2-layer MLP with the MNIST dataset, 16bit fixed precision can be used to achieve the same accuracy as floating point if stochastic rounding is used.  For rounding with precision of $\epsilon = 2^{-FL}$ where FL is the number of decimal bits, stochastic rounding rounds up or down randomly with probability proportional to the distance between $\lfloor{x}\rfloor$ and $\lfloor{x}\rfloor + x$.  Here, $\lfloor{x}\rfloor$ is the closest integer multiple of $\epsilon$.  

\begin{align*}
round(x) = 
\begin{cases}
\lfloor{x}\rfloor, & w.p. 1-\frac{x-\lfloor{x}\rfloor}{\epsilon}\\
\lfloor{x}\rfloor + \epsilon, & w.p. \frac{x-\lfloor{x}\rfloor}{\epsilon}
\end{cases}
\end{align*}


==> intro-copy-copy.tex <==
\section{Introduction}

State of the art Deep Neural Networks (DNNs) are becoming deeper and can be applied to a range of sophisticated cognitive tasks such as image recognition~\cite{cnn} and natural language processing~\cite{rnn}. Convolutional Neural Networks (CNNs)~\cite{cnn} and Recurrent Neural Networks (RNNs)~\cite{rnn} are some of the commonly used network architectures that are inspired by the Multilayer Perceptron (MLP)~\cite{mlp}. Most of the community has focused on acceleration of the forward path/inference for DNNs, neglecting the acceleration for training~\cite{SzeSurvey,TPU}. Training DNNs is a performance and energy costly operation that routinely takes weeks or longer on servers~\cite{gpu}. This makes the task of navigating the hyper parameter space for network architecture expensive. However the nature of computation in training DNNs makes it an excellent candidate for specialized acceleration if the necessary computation/communication functionality is supported~\cite{sys_array}. 

Today, acceleration of the training process is primarily done on GPUs~\cite{gpu}. However, GPUs suffer from fundamental computation, memory, and bandwidth imbalance in their memory hierarchy~\cite{TPU}. Thus, the fundamental question is what are the compute architecture, memory hierarchy, and algorithmic trade-offs for an accelerator designed to train deep neural networks. In this paper we aim to address the design tradeoffs by introducing a Coarse Grain Reconfigurable Architecture (CGRA) for training MLPs.

We  focus on training MLPs, an important class of networks currently used on state of the art servers~\cite{TPU}, with several variants of backpropagation (BP)~\cite{bp}. Although the computation and the communication graph for CNNs and RNNs are more complex compared to MLPs, we chose MLPs because of the following reasons. First, MLPs are inherently memory bound operation and harder to accelerate. Second, several research studies on the principles of BP and optimization in DNNs investigate MLPs because of their simpler network architecture~\cite{dfa_results,stochastic,hogwild}. Finally, MLPs represent the fully-connected layers of CNNs~\cite{cnn}. We believe this effort establishes a platform for future work on training CNNs and RNNs.

\begin{comment}
We focus on several variants of backpropagation (BP)~\cite{bp}, which is the standard optimization method used to train arbitrary DNNs.  Although the computation and the communication graph for CNNs and RNNs are more complex compared to MLPs, several research studies on the principles of BP and optimization in DNNs investigate MLPs because of their simpler network architecture~\cite{dfa_results,stochastic,hogwild}.  They also represent the fully-connected layers of CNNs~\cite{cnn} and are memorybound. Therefore, this effort establishes a platform for future work on training CNNs and RNNs.
\end{comment}

The challenge in training DNNs is that the fastest converging gradient descent algorithms in terms of passes over the dataset are not efficient in conventional architectures as they are based on General Matrix-Vector Multiplication (GEMV), which is a bandwidth limited operation. For sparse network weights, sparse matrix-vector multiplication is even less compute intensive, however as the size of the network shrinks and is able to fit on local storage, the overall cost of communication drops.~\cite{spmv}.  GPUs use a variant that groups samples into batches in order to overcome bandwidth limitations at the cost of more epochs to convergence and perform General Matrix-Matrix Multiplication (GEMM), which is a compute intensive kernel. 

Given the fundamental differences in various techniques for training MLPs, we aim to compare the design space of accelerators and the memory hierarchy for various configurations of networks and training algorithms. This paper makes the following contributions:

\begin{figure}[!t]
\vspace{-15pt}
\centering
\includegraphics[width=0.25\textwidth]{mlp_diagram.png}
\vspace{-10pt}
\caption{An MLP with 2 hidden layers $h_1$ and $h_2$}
\vspace{-15pt}
\label{fig:mlp_diagram}
\end{figure}



\begin{figure*}[!pt]
\centering
\vspace{-20pt}
\includegraphics[width=.8 \textwidth]{NetworkU}
\vspace{-10pt}
\caption{Methods of learning. Each arrow demonstrates one sample's movement through the forward and backward path in time. (a) SGD, (b) MBGD, (c) DFA, (d), CP}
\vspace{-10pt}
\label{fig:learning}
\end{figure*}



\begin {itemize}
\setlength{\itemindent}{.1em}
\item Techniques to decrease dependencies, and increase locality and parallelism for training DNNs and their effect on convergence.
\item Exploration of the design space of accelerators for various BP algorithms.
\item CATERPILLAR: an efficient architecture targeting both GEMV and GEMM optimized for fast collective communications and training DNNs.
\item Evaluation of the costs of convergence of various networks/algorithms/accelerators with respect to both performance and energy efficiency.

\end{itemize}

The rest of the paper is organized as follows: Section~\ref{sec:related} reviews related work in architectures. Section~\ref{sec:mlp} describes algorithms for training DNNs.  Section~\ref{sec:architecture} discusses the proposed CGRA, and the mapping tradeoffs.  Section~\ref{sec:results} presents the experimental results.  Finally, Section ~\ref{sec:conclusion} presents conclusions and future work.

%\hfill mds
 
%\hfill August 26, 2015


